The Patterns of Life Human Mobility Simulation

We demonstrate the Patterns of Life Simulation to create realistic simulations of human mobility in a city. This simulation has recently been used to generate massive amounts of trajectory and check-in data. Our demonstration focuses on using the simulation twofold: (1) using the graphical user interface (GUI), and (2) running the simulation headless by disabling the GUI for faster data generation. We further demonstrate how the Patterns of Life simulation can be used to simulate any region on Earth by using publicly available data from OpenStreetMap. Finally, we also demonstrate recent improvements to the scalability of the simulation allows simulating up to 100,000 individual agents for years of simulation time. During our demonstration, as well as offline using our guides on GitHub, participants will learn: (1) The theories of human behavior driving the Patters of Life simulation, (2) how to simulate to generate massive amounts of synthetic yet realistic trajectory data, (3) running the simulation for a region of interest chosen by participants using OSM data, (4) learn the scalability of the simulation and understand the properties of generated data, and (5) manage thousands of parallel simulation instances running concurrently.

==> content/results.tex <==

As described in \refsec{sec:methodology}, we improved the performance of the Vanilla version by optimizing different aspects of the simulation, such as distance calculation and logging system. The Emory version can run faster than the Vanilla version due to these optimizations. 

% \subsection{Generated Data}

% We generated an example dataset using the Emory version of the simulation. The dataset consists of 10,000 agents and 2,880,000 location observations. The data for an example day is visualized in \reffig{fig:generated_data}. The data wrangling mechanism were used to clean and pre-process the data in~\cite{amiri2023massive}.

% \begin{figure}
%     \centering
%     \includegraphics[trim = 2cm 2cm 2cm 2cm, clip, width=1\linewidth]{figs/generated_data.png}
%     \vspace{-0.451cm}
%     \caption{ Simulation on 2020-01-01 10K Agents and 2,880,000 Location Observations} \vspace{-0.451cm}
%     \label{fig:generated_data}
%     \vspace{-0.451cm}
% \end{figure}

==> content/scenario.tex <==




% \begin{figure}[!ht]
%     \centering

%     \begin{verbatim}

% java -Dlog4j2.configurationFactory=
% edu.emory.amiri.life.log.CustomConfigurationFactory
% -Dlog.rootDirectory=logs -Dsimulation.test=c01 
% -jar ../jar/life.jar -configuration modified.properties 
% -until 2880
%     \end{verbatim}
%     \vspace{-0.7cm}
%     \caption{An example of an execution command to run the \texttt{life.jar} file with the \texttt{c01} logging option for 2880 simulation ticks, equivalent to 10 days.}
%     \label{fig:java_command}
% \end{figure}


%\textcolor{red}{This seems to be too much detail for a demo paper:
%In greater detail, we will focus on headless execution, an optimal method for data generation that can be implemented on any machine equipped with Java. We will illustrate how to alter the simulation's source code to integrate custom features and subsequently compile this modified code into a JAR file. Using a Bash script on Linux, we will demonstrate a use case that involves running a single simulation instance with predefined parameters to showcase the data generation process for that instance. Furthermore, we will explore the creation and customization of log files during this stage, using both the simulation source code and the provided data processing scripts.
%To initiate a single instance of the simulation, the Java command is encapsulated within a Bash file named \texttt{run.sh}. Executing  \texttt{bash run.sh} activates the command. Users can customize logging options to specify the details to be recorded, as well as set the number of ticks for data generation. Each tick's interval is defined as an input parameter; the default interval is 5 minutes. This setting ensures that every five minutes, corresponding to simulation time, the simulation progresses to the subsequent step and verifies the step requirements. By maintaining each interval at 5 minutes, a day within the simulation consists of 288 ticks, which should be detailed as an input arguments in the Java command. The agent's log information can be adjusted within the simulation's logging channel, and the output logs will be stored in a folder named \texttt{logs}.
%}

% \begin{figure}
%     \centering
%     \begin{verbatim}
% [{"properties": {
%     "numOfAgents": 182,
%     "maps": "../maps/atl/map/"},
% "id": "id_t01",
% "config": {
%     "run_sh_path": "/../id_t01/run.sh"},
% "status": "pending"}]
% \end{verbatim}
%     \vspace{-0.451cm}
%     \caption{An example of a JSON entry for parameterization of the simulation.}
%     \vspace{-0.451cm}
%     \label{fig:json_parammeter}
% \end{figure}

\begin{figure}
    \centering
    \begin{verbatim}
initialized = get_initial_parameters()
configured = get_configured_params(initialized)
simulated = run(configured,fork_join=False,parallel=8)
save_params(simulated,f"params.simulated.json")
\end{verbatim}
    % \vspace{-0.452cm}
    \caption{An example of a Python script to run multiple simulation instances in parallel.}%\vspace{-0.452cm}}

    \label{fig:run_parallel}
    % \vspace{-0.309452cm}
\end{figure}
After introducing the simulation and data generation processes, we will utilize the developed framework to execute multiple simulation instances. This involves initially configuring the instances and then running them. We will demonstrate that both fork-join and job-queue models can be employed during this phase. The fork-join model is optimal for parallel execution with dependencies, such as when parameters need to be tuned in a genetic algorithm. Conversely, the job-queue model uses a queue to manage instances, allowing for parallel execution without dependencies. The number of parallel instances can be adjusted according to the machine's capacity.
%
To configure the instances, users can employ a JSON format for parameters in which properties are the parameters for the simulation, equivalent to parameters.properties in the Vanilla version. While creating the JSON file to configure the simulations, users can specify the run path. They can then choose between the fork-join and job-queue models to run the instances in parallel using  Python scripts.
In \reffig{fig:run_parallel}, the provided Python script illustrates the process of running multiple simulation instances concurrently. Initially, the script fetches the default parameters using \textit{get\_initial\_parameters()} function. Subsequently, these parameters are configured through \textit{get\_configured\_params()}. The \textit{run()} function then executes the simulation with the configured parameters, enabling parallel processing by setting fork\_join to \textit{False} and specifying eight parallel processes. Finally, the meta data of the simulations are stored in a JSON file, \textit{params.simulated.json}, for further analysis or reuse. This script exemplifies an efficient method for managing and executing simulations in a parallel computing environment, optimizing computational resources and reducing the overall execution time. Notably, this parallel execution method does not affect an individual simulation's performance, as each simulation instance is executed independently and concurrently, ensuring that the results are accurate and reliable; this is particularly beneficial for large-scale data generation and research applications.



After data generation, the logs from each simulation can be processed in two ways: by concatenating the logs from each instance or by selectively trimming and concatenating logs from a subset of the parallel instances. This stage demonstrates how the simulated data can be utilized in various applications, such as training machine learning algorithms. We developed a Python script that processes these logs to produce the final dataset for analysis. For instance, \textit{agentStateTable} log file might be split into smaller files. This table records the agent's state at each simulation tick. The script then concatenates the logs from each instance, producing a consolidated dataset for further processing. Users can also customize which columns to include in the final dataset. This script is designed for flexibility and customizability, enabling users to adapt data processing to meet specific research needs. Through a detailed demonstration of the simulation, data generation, and data processing steps, we aim to highlight the framework’s capability and adaptability for a variety of research and commercial applications.
%
\textbf{\textit{A comprehensive documentation of the framework and its functionalities are available on the GitHub repository that shows how to run the simulation, generate data, and process the logs for further analysis.}}



